Active Representation Learning for General Task Space with Applications in Robotics

Representation learning based on multi-task pretraining has become a powerful approach in many domains. In particular, task-aware representation learning aims to learn an optimal representation for a specific target task by sampling data from a set of source tasks, while task-agnostic representation learning seeks to learn a universal representation for a class of tasks. In this paper, we propose a general and versatile algorithmic and theoretic framework for \textit{active representation learning}, where the learner optimally chooses which source tasks to sample from. This framework, along with a tractable meta algorithm, allows most arbitrary target and source task spaces (from discrete to continuous), covers both task-aware and task-agnostic settings, and is compatible with deep representation learning practices. We provide several instantiations under this framework, from bilinear and feature-based nonlinear to general nonlinear cases. In the bilinear case, by leveraging the non-uniform spectrum of the task representation and the calibrated source-target relevance, we prove that the sample complexity to achieve $\varepsilon$-excess risk on target scales with $ (k^*)^2 \|v^*\|_2^2 \varepsilon^{-2}$ where $k^*$ is the effective dimension of the target and $\|v^*\|_2^2 \in (0,1]$ represents the connection between source and target space. Compared to the passive one, this can save up to $\frac{1}{d_W}$ of sample complexity, where $d_W$ is the task space dimension. Finally, we demonstrate different instantiations of our meta algorithm in synthetic datasets and robotics problems, from pendulum simulations to real-world drone flight datasets. On average, our algorithms outperform baselines by $20\%-70\%$.

==> Results1-CubeSpace/Algorithm.tex <==

\subsection{Algorithms}
\begin{algorithm}[H]
\caption{Algorithm for cubic source space with fixed non-overlap single target $w_0$}
\label{algo: main}
\begin{algorithmic}[1]
\STATE \textbf{Inputs.} Candidate source set of task parameter $\calW_\text{source}$ and a target task $w_0 \perp \calW_\text{source}$
\STATE \textbf{Other Inputs:} Sampling oracle Inputs, Budget limitations, Candidate model inputs. (Skip here)
\STATE Set initial sampling distribution $q_0$ to help find the exploration basis as
\begin{align*}
    q_0(e_t) = \frac{1}{d_W}, \forall t \in d_W, \quad \text{and} \quad q_0(w) = 0 \text{ otherwise}
\end{align*}
\STATE Set $n_0 = k^2 d_X \kappa^6(B_W)$ and collect $n_0$ data for each task denoted as $\{X_w\}_{w=e_1,e_2,\ldots, e_{d_W}, e_{d_W+1}}$
\STATE Update $\hat{B}_X^0 \leftarrow \calO_\text{base 1}^X$ and $\hat{B}_W^0 \leftarrow \calO_\text{base}^W$ 
\STATE Compute the \textit{exploration} sampling distribution $q_1$ as the solution of
\begin{align*}
    q_1(v_i) = \frac{1}{k}, \forall i \in k, \quad \text{and } q_0(w) = 0 \text{ otherwise} 
\end{align*}
\text{Here} $v_i$ is the $i$-th of $V$ and $\_,\_,V \leftarrow \text{SVD}(\hat{B}_W^0 \left( I_{d_W+1} - \frac{w_0 w_0^\top}{\|w_0\|_2^2} \right))$
\FOR{$j = 1,2,3, \ldots$}
    \STATE Set $n_t \approx q_1(w) \epsilon^{-\frac{3}{2}}$ \textcolor{red}{Other dependence?}
    \STATE Collecting $n_t$ for each task $v_i$ and update data $\{X_w\}_{w | q_1(w) \neq 0 }$
    \STATE Update $\hat{B}_X^{j} \leftarrow \calO_\text{base 2}^X$ and $\hat{B}_W^j \leftarrow \calO_\text{base}^W$ 
    \STATE Find the exploitation task parameterized by 
    \begin{align*}
        \Tilde{w}_j = \text{Proj}_{\calW_\text{source}} w' =
        \begin{cases}
            &  \frac{w'}{\|w'\|_2} \text{when } \calW_\text{source} = [-1,1]^{d_W} \\
            &  \frac{w'}{\|w'\|_\infty} \quad \text{when } \calW_\text{source} = \fB^{d_W}(1)
        \end{cases}
    \end{align*}
    where
    \begin{align*}
       & w' = 
        \begin{cases}
            & \argmin_{w} \|w\|_2 \quad \text{when } \calW_\text{source} = [-1,1]^{d_W} \\
            & \argmin_{w} \|w\|_\infty \quad \text{when } \calW_\text{source} = \fB^{d_W}(1)
        \end{cases}\\
        &\text{s.t.} \quad \hat{B}_W^j w = \hat{B}_W^j w_0
    \end{align*}
    \STATE Assign $\tilde{n}$ sampling budget to task parameterized by $\tilde{w}_j$ where
    \begin{align*} 
        \tilde{n} 
        \approx
        \frac{ \|\hat{B}_W^j w_0\|_2}{ \|\hat{B}_W^j \tilde{w}_j \|_2}
        =
        \begin{cases}
            & \frac{1}{\epsilon^2}* \tilde{\beta} \|w'\|_2^2 \quad \text{when } \calW_\text{source} = [-1,1]^{d_W} \\
            & \frac{1}{\epsilon^2}* \tilde{\beta} \|w'\|_0^2 \quad \text{when } \calW_\text{source} = \fB^{d_W}(1)
        \end{cases}
        \quad \text{and} \quad \tilde{\beta} = 8 
    \end{align*}
    \STATE Collecting and update data $X_{\tilde{w}_j}$
    \STATE Update $\tilde{B}_X^j, \tilde{B}_w^j$ as the solution of ERM
\ENDFOR
\STATE \textbf{Return }  $\tilde{B}_X^j, \tilde{B}_w^j$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[H]
\caption{Algorithm for cubic source space with fixed target distribution $\nu_0$}
\label{algo: main}
\begin{algorithmic}[1]
\STATE \textbf{Inputs.} Candidate source and target set of task parameter $\calW_\text{source}, \calW_\text{target}$ and a target task distribution $\nu_0 \in \Delta(\calW_\text{target})$
\STATE \textbf{Other Inputs:} Sampling oracle Inputs, Budget limitations, Candidate model inputs. (Skip here)
\STATE Set initial sampling distribution $q_0$ to help find the exploration basis as
\begin{align*}
    q_0(e_t) = \frac{1}{d_W}, \forall t \in d_W, \quad \text{and} \quad q_0(w) = 0 \text{ otherwise}
\end{align*}
\STATE Set $n_0 = \textcolor{red}{pending}$ and collect $n_0$ data for each task denoted as $\{X_w\}_{w=e_1,e_2,\ldots, e_{d_W}, e_{d_W+1}}$
\STATE Update $\hat{B}_X^0 \leftarrow \calO_\text{base 1}^X$ and $\hat{B}_W^0 \leftarrow \calO_\text{base}^W$ 
\STATE Compute the \textit{exploration} sampling distribution $q_1$ as the solution of
\begin{align*}
    q_1(v_i) = \frac{1}{k}, \forall i \in k, \quad \text{and } q_0(w) = 0 \text{ otherwise} 
\end{align*}
\text{Here} $v_i$ is the $i$-th of $V$ and $U,D,V \leftarrow \text{SVD}(\hat{B}_W^0 - {\color{red}proj?})$
\FOR{$j = 1,2,3, \ldots$}
    \STATE Set $n_1^j \approx q_1(w) \epsilon^{-\frac{3}{2}}$ \textcolor{red}{Other dependence?}
    \STATE Collecting $n_t$ for each task $v_i$ and update data $\{X_w\}_{w | q_1(w) \neq 0 }$
    \STATE Update $\hat{B}_X^{j} \leftarrow \calO_\text{base 2}^X$ and $\hat{B}_W^j \leftarrow \calO_\text{base}^W$ 
    \STATE Find a set of exploitation tasks parameterized by $\Tilde{W}_j$ with each column $i$ as
    \begin{align*}
        \Tilde{W}_j(i) = \text{Proj}_{\calW_\text{source}} w_i^\prime =
        \begin{cases}
            &  \frac{w_i^\prime}{\|w_i^\prime\|_2} \text{when } \calW_\text{source} = [-1,1]^{d_W} \\
            &  \frac{w_i^\prime}{\|w_i^\prime\|_\infty} \quad \text{when } \calW_\text{source} = \fB^{d_W}(1)
        \end{cases}
    \end{align*}
    where
    \begin{align*}
        \text{i-th column of } W' = 
        &w_i^\prime = 
        \begin{cases}
            & \argmin_{w} \|w\|_2 \quad \text{when } \calW_\text{source} = [-1,1]^{d_W} \\
            & \argmin_{w} \|w\|_\infty \quad \text{when } \calW_\text{source} = \fB^{d_W}(1) 
        \end{cases} \\
        \text{s.t.} \quad & \hat{B}_W^j w =  u_i\sqrt{\lambda_i} \quad {\color{red} \forall \Lambda_i \geq ?}\\
        & \text{where } U, \Lambda \leftarrow  \text{Eig}\left(\E_{w_0 \sim \nu_0}\left[\hat{B}_W^j  w_0 (\hat{B}_W^j w_0)^\top \right] \right)
    \end{align*}
    \STATE Compute the \textit{exploitation} sampling distribution $\tilde{q}_j$ as the solution of
    \begin{align*}
        \tilde{q}_j(w) = \frac{1}{\text{\# col}(\tilde{W}_j)}, \forall w \in \text{col}(\Tilde{W}_j), \quad \text{and } \tilde{q}_j(w) = 0 \text{ otherwise} 
    \end{align*}
    % \STATE Assign $\tilde{n}(w) \approx \frac{\tilde{q}_j(w)}{\text{\# col}(\tilde{W}_j)\epsilon^2}* {\color{red}\tilde{\beta}} \frac{\trace\left( \hat{B}_W^j W' \right)}{\trace\left( \hat{B}_W^j \text{Proj}_{\calW_\text{source}} W' \right)} $ sampling budget to each task parameterized by each column of $\Tilde{W}_j$ 
    \STATE Assign $\tilde{n}$ sampling budget to tasks parameterized by $\tilde{W}_j$ where
    \begin{align*} 
        \tilde{n}(w)
        &=\frac{\tilde{q}_j(w)}{\epsilon^2} * \text{\# col}(\tilde{W}_j)\tilde{\beta} \max_i \frac{\Lambda_i}{\|\hat{B}_W^j \tilde{W}_j(i)\|_2^2} \\
        &= 
        \begin{cases}
            & \frac{\tilde{q}_j(w)}{\epsilon^2} * \text{\# col}(\tilde{W}_j)\tilde{\beta} \max_i \|W_j^\prime(i)\|_2^2 \quad \text{when } \calW_\text{source} = [-1,1]^{d_W} \\
            & \frac{1}{\epsilon^2} * \text{\# col}(\tilde{W}_j)\tilde{\beta} \max_i \|W_j^\prime(i)\|_\infty^2  \quad \text{when } \calW_\text{source} = \fB^{d_W}(1)
        \end{cases}
    \end{align*}
    \STATE Collecting and update data $\{X_w\}_{w \in \text{col}(\Tilde{W}_j)}$
    \STATE Update $\hat{B}_X, \hat{B}_W$ as 
\ENDFOR
\STATE \textbf{Return }  $\tilde{B}_X^j, \tilde{B}_w^j$
\end{algorithmic}
\end{algorithm}

Notice that this explicit solution is one of the feasible solutions under the following general version (Algo.~\ref{algo: main-general}). Specifically, we have for any epoch $j$,
\begin{align*}
    & \min_{q} \lambda_{max}\left( \left( \sum_{w} q (\hat{B}_j w)(\hat{B}_j w)^\top \right)^{-1} \E_{w_0}\left[(\hat{B}_j w)(\hat{B}_j w)^\top \right] \right) \\
    & \leq \lambda_{max}\left( \left( \sum_{w} \tilde{q}_j (\hat{B}_j w)(\hat{B}_j w)^\top \right)^{-1} \E_{w_0}\left[(\hat{B}_j w)(\hat{B}_j w)^\top \right] \right) \\
    &=  \max_i \frac{\Lambda_i}{\|\hat{B}_W^j \tilde{W}_j(i)\|_2^2} 
    =  \begin{cases}
            &  \text{\# col}(\tilde{W}_j) \max_i \|\tilde{W}_j(i)\|_2^2 \quad \text{when } \calW_\text{source} = [-1,1]^{d_W} \\
            &  \text{\# col}(\tilde{W}_j) \max_i \|\tilde{W}_j(i)\|_\infty^2  \quad \text{when } \calW_\text{source} = \fB^{d_W}(1)
        \end{cases}
\end{align*}

\begin{algorithm}[H]
\caption{A more general version}
\label{algo: main-general}
\begin{algorithmic}[1]
\STATE \textbf{Inputs.} Candidate source and target set of task parameter $\calW_\text{source}, \calW_\text{target}$ and a target task distribution $\nu_0 \in \Delta(\calW_\text{target})$
\STATE \textbf{Other Inputs:} Sampling oracle Inputs, Budget limitations, Candidate model inputs. (Skip here)
\STATE Set initial sampling distribution $q_0$ to help find the exploration basis as
\begin{align*}
    q_0(e_t) = \frac{1}{d_W}, \forall t \in d_W, \quad \text{and} \quad q_0(w) = 0 \text{ otherwise}
\end{align*}
\STATE Set $n_0 = \textcolor{red}{pending}$ and collect $n_0$ data for each task denoted as $\{X_w\}_{w=e_1,e_2,\ldots, e_{d_W}, e_{d_W+1}}$
\STATE Update $\hat{B}_X^0 \leftarrow \calO_\text{base 1}^X$ and $\hat{B}_W^0 \leftarrow \calO_\text{base}^W$ 
\STATE Compute the \textit{exploration} sampling distribution $q_1$ as the solution of
\begin{align*}
    q_1(v_i) = \frac{1}{k}, \forall i \in k, \quad \text{and } q_0(w) = 0 \text{ otherwise} 
\end{align*}
\text{Here} $v_i$ is the $i$-th of $V$ and $U,D,V \leftarrow \text{SVD}(\hat{B}_W^0 - {\color{red}proj?})$
\FOR{$j = 1,2,3, \ldots$}
    \STATE Set $n_1^j \approx q_1(w) \epsilon^{-\frac{3}{2}}$ \textcolor{red}{Other dependence?}
    \STATE Collecting $n_t$ for each task $v_i$ and update data $\{X_w\}_{w | q_1(w) \neq 0 }$
    \STATE Update $\hat{B}_X^{j} \leftarrow \calO_\text{base 2}^X$ and $\hat{B}_W^j \leftarrow \calO_\text{base}^W$ 
    \STATE Compute the \textit{exploitation} sampling distribution $\tilde{q}_j$ as the solution of
    \begin{align*}
        \min_{q \in \Delta(\calW_\text{source})} \lambda_{\max} \left( \left(\sum_{w \in \calW_\text{source}} q(w) \hat{B}_j w (\hat{B}_j w)^\top \right)^{-1}  \Sigma_\gamma  \right)
    \end{align*}
    where $\Sigma_\gamma = \text{clip}(\hat{B}_j\E_{w_0 \sim \nu_0} w_0 w_0^\top\hat{B}_j^\top, \gamma)$. \\
    Denote the collection of sampled target as $\tilde{W}_j$ satisfies $\sum_{w \in \calW_\text{source}} q(w) w w^\top = \tilde{W}_j\tilde{W}_j^\top$.
    \STATE Assign $\tilde{n}$ sampling budget to tasks parameterized by $\tilde{W}_j$ where
    \begin{align*} 
        \tilde{n}(w)
        & =\frac{\tilde{q}_j(w)}{\epsilon^2} * \Tilde{\beta} \lambda_{\max} \left( \left(\sum_{w \in \calW_\text{source}} \tilde{q}_j(w) \hat{B}_j w (\hat{B}_j w)^\top \right)^{-1}  \Sigma_\gamma  \right)
    \end{align*}
    Denote $W'$ satisfies $ \lambda_{\max} \left( \left(\sum_{w \in \calW_\text{source}} \tilde{q}_j(w) \hat{B}_j w (\hat{B}_j w)^\top \right)^{-1}  \Sigma_\gamma  \right) \Tilde{W}_j\Tilde{W}_j^\top = W' (W')^\top$
    \STATE Collecting and update data $\{X_w\}_{w \in \text{col}(\Tilde{W}_j)}$  
    \STATE Update $\hat{B}_X, \hat{B}_W$ as 
\ENDFOR
\STATE \textbf{Return }  $\tilde{B}_X^j, \tilde{B}_w^j$
\end{algorithmic}
\end{algorithm}


==> Results1-CubeSpace/Analysis-Stage0.tex <==
\subsection{Guarantees for the exploration basis}


\subsubsection{Important Lemmas}
By abusing the notation a little bit, we denote $\hat{B}_W^0$ here as the one projected to $\calW_\text{source}$.

\begin{lemma}[Guarantee on exploration basis 1]
\yifang{Maybe just say $\hat{B}_W$, Clean the notation for spectral norm}
\yifang{no c need}
\label{lem: helper base est}
    For some arbitrary matrix $M_3$, suppose there exists
    \begin{align*}
        & 8c \| B_W - c \hat{B}_W^0\| \|B_W \|_2  \|M_3\| \leq \frac{1}{2}\lambda_{\min}(B_W M_3 B_W^\top), \quad \text{for some arbitrary constant } c \\
        & \{v_i\}_{i=1}^k \leftarrow \text{column space of }\textsc{SVD}(\hat{B}_W^0),
    \end{align*}
    then we have, 
    \begin{align*}
        \frac{1}{2}  B_W M_3 (B_W)^\top
        \leq B_W\left(\sum_{i=1}^k v_i v_i^\top \right) M_3 \left(\sum_{i=1}^k v_i v_i^\top \right) (B_W)^\top
        \leq  \frac{3}{2} B_W M_3 (B_W)^\top,
    \end{align*}
\end{lemma}
\begin{proof}
    \begin{align*}
        &\left(B_W \sum_{i=1}^k v_i v_i^\top \right)^\top  M_3 \left(B_W \sum_{i=1}^k v_i v_i^\top \right) - B_W M_3 (B_W)^\top \\
        & = B_W\left(\sum_{i=1}^k v_i v_i^\top \right)  M_3 \left(\sum_{i=1}^k v_i v_i^\top \right) B_W^\top 
            - c^2 \hat{B}_W^0 \left(\sum_{i=1}^k v_i v_i^\top \right) M_3 \left(\sum_{i=1}^k v_i v_i^\top \right) (\hat{B}_W^0)^\top \\
            & \quad + c^2 \hat{B}_W^0 \left(\sum_{i=1}^k v_i v_i^\top \right) M_3 \left(\sum_{i=1}^k v_i v_i^\top \right) (\hat{B}_W^0)^\top - B_W M_3 B_W^\top \\
        & = B_W\left(\sum_{i=1}^k v_i v_i^\top \right)  M_3 \left(\sum_{i=1}^k v_i v_i^\top \right) B_W^\top 
            - c^2 \hat{B}_W^0 \left(\sum_{i=1}^k v_i v_i^\top \right) M_3 \left(\sum_{i=1}^k v_i v_i^\top \right) (\hat{B}_W^0)^\top \\
            & \quad + c^2 \hat{B}_W^0 M_3  (\hat{B}_W^0)^\top - B_W M_3 B_W^\top \\
        & = (B_W - c \hat{B}_W^0)  \left(\sum_{i=1}^k v_i v_i^\top \right)M_3 \left(\sum_{i=1}^k v_i v_i^\top \right) B_W^\top 
            + c \hat{B}_W^0 \left(\sum_{i=1}^k v_i v_i^\top \right)M_3 \left(\sum_{i=1}^k v_i v_i^\top \right) (B_W - c \hat{B}_W^0)^\top \\
            & \quad + c (c \hat{B}_W -  B_W) M_3 (\hat{B}_W^0)^\top + B_W M_3 (c \hat{B}_W^0 -  B_W)^\top
    \end{align*}
    The last equality comes from the definition of $v_i$. We can further upper bound its spectral norm by 
    \begin{align*}
        2 \| B_W - c \hat{B}_W\| 
        \left(c \|\hat{B}_W\|_2 + \|B_W\|_2\right) \|M_3\|
        & \leq 4c \| B_W - c \hat{B}_W^0\| \|B_W \|_2 \|M_3\| +  2c \| B_W - \hat{B}_W^0\|_2^2 \|M_3\| \\
        & \leq 8c \| B_W - c \hat{B}_W^0\| \|B_W \|_2 \|M_3\|
    \end{align*}
    Therefore, by the definition of spectral norm, we can get 
    \begin{align*}
        & B_W \left(\sum_{i=1}^k v_i v_i^\top \right) (B_W)^\top - B_W (B_W)^\top
        \leq   8c \| B_W - c \hat{B}_W\| \|B_W \|_2  \|M_3\| I_k \\
        & B_W \left(\sum_{i=1}^k v_i v_i^\top \right) (B_W)^\top - B_W (B_W)^\top
        \geq  - 8c \| B_W - c \hat{B}_W\| \|B_W \|_2  \|M_3\| I_k
    \end{align*}
    Given the upper bound on $8c \| B_W - c \hat{B}_W\| \|B_W \|_2  \|M_3\|$, we get the final bound.
    \begin{align*}
        8 \| B_W - \hat{B}_W^0\| \|B_W \|_2  \|M_3\| I_k
        \leq \lambda_{\min}(B_W M_3 B_W^\top) I_k
        \leq B_W M_3 B_W^\top
    \end{align*}
\end{proof}



\textbf{Now we are ready to prove the main lemma to show that this estimated exploration basis is enough.}
\yifang{Maybe add trace to remove the $M_3$? And use notation $\dot{B}$}
\begin{lemma}[Main: basic estimation lemma]
\label{lem: main base est}
    Suppose there the estimated $\hat{B}_W^0$ satisfies for some arbitrary $M_3$
    \begin{align*}
        \frac{1}{2}  B_W M_3 (B_W)^\top
        \leq B_W\left(\sum_{i=1}^k v_i v_i^\top \right) M_3 \left(\sum_{i=1}^k v_i v_i^\top \right) (B_W)^\top
        \leq  \frac{3}{2} B_W M_3 (B_W)^\top,
    \end{align*}
    then by computing $\hat{B}_W$ as \yf{Notation?}
    $
    \hat{B}_W = \argmin_{B_W \in \fR^{d_W \times k}} \left(\|X_0 \hat{B}_X^\top B_W w_0  - Y_0\|_2  + \sum_{i=1}^k \|X_w  \hat{B}_X^\top B_W v_i - Y_w\|_2 \right),
    $
    we have
    \begin{align*}
         & \hat{B}_W M_3 \hat{B}_W^\top \leq 2\kappa_X M_1 B_W  M_3  B_W^\top M_1^\top+ \text{Noise},
         & -\hat{B}_W  M_3  \hat{B}_W^\top \leq - \frac{1}{4}\frac{1}{\kappa_X} M_1 B_W  M_3  B_W^\top M_1^\top - \text{Noise}
    \end{align*}
\end{lemma}
where 
\begin{align*}
    & M_1 =\left(\hat{B}_X \hat{B}_X^\top\right)^{-1} \hat{B}_X  B_X^\top\\
    & \text{Noise} = \sum_{i} M_i^2 \xi_i M_3 \xi_i^\top  (M_i^2)^\top
                + \sum_{i} M_{i,1} B_W v_i v_i^\top  M_3 \xi_i^\top (M_{i,2})^\top
                + \sum_{i}  M_{i,2} \xi_i M_3 v_i v_i^\top B_W^\top (M_{i,1})^\top\\
    & M_{i,2} = \left(\hat{B}_X X_i^\top X_i \hat{B}_X^\top\right)^{-1} \hat{B}_i X_i^\top
\end{align*}
\begin{proof}
    From \cite{chen2022active}, we get that the explicit form of $\hat{w}(w)$, which is the estimation of actual $B_W w$ as
    \begin{align*}
        \underbrace{\left(\hat{B}_X X_w^\top X_w \hat{B}_X^\top\right)^{-1} \hat{B}_X X_w^\top X_w B_X^\top}_{M_{w,1}} B_W w
            + \underbrace{\left(\hat{B}_X X_w^\top X_w \hat{B}_X^\top\right)^{-1} \hat{B}_W X_w^\top}_{M_{w,2}} \xi_w
    \end{align*}
    By abusing notation a little bit, here we use subscription $i$ to denote the items that associate the task encoded by $v_i$. Therefore, we have 
    % \begin{align*}
    %     \hat{B}_W = & \sum_{i=1}^m \hat{w}(v_i) v_i 
    %         =  \sum_{i} M_{i,1} B_W v_iv_i^\top
    %         + \sum_{i} M_{i,2} \xi_i v_i^\top \\
    %    \hat{B}_W M_3 \hat{B}_W^\top
    %      & = \left(\sum_{i} M_{i,1} B_W v_iv_i^\top \right) M_3  \left(\sum_{i} M_{i,1} B_W v_iv_i^\top \right)^\top\\
    %         & + \underbrace{\sum_{i}M_{i,2}^2 \xi_i M_3 \xi_i^\top  (M_{i,2}^2)^\top
    %             + \sum_{i} M_{i,1} B_W v_i v_i^\top  M_3 \xi_i^\top (M_{i,2})^\top
    %             + \sum_{i}  M_{i,2} \xi_i M_3 v_i v_i^\top B_W^\top (M_{i,1})^\top}_\text{Noise}\\
    %     & \leq \frac{1.1}{0.9} \kappa_X M_1 B_W (\sum_{i} v_iv_i^\top) M_3 (\sum_{i} v_iv_i^\top) B_W^\top M_1^\top + \text{Noise}\\
    %     \hat{B}_W \hat{B}_W^\top
    %     & \geq \frac{0.9}{1.1} \frac{1}{\kappa_X} M_1 B_W (\sum_{i} v_iv_i^\top) M_3 (\sum_{i} v_iv_i^\top) B_W^\top M_1^\top + \text{Noise}
    % \end{align*}
    \begin{align*}
        \hat{B}_W = & \sum_{i=1}^m \hat{w}(v_i) v_i 
            =  \sum_{i} M_{i,1} B_W v_iv_i^\top
            + \sum_{i} M_{i,2} \xi_i v_i^\top \\
       \hat{B}_W M_3 \hat{B}_W^\top
         & = \left(\sum_{i} M_{i,1} B_W v_iv_i^\top \right) M_3  \left(\sum_{i} M_{i,1} B_W v_iv_i^\top \right)^\top\\
            & + \underbrace{(\sum_{i}M_{i,2} \xi_i v_i^\top) M_3 (\sum_{i}M_{i,2} \xi_i v_i^\top)^\top
                + (\sum_{i} M_{i,1} B_W v_i v_i^\top)  M_3 (\sum_{i}M_{i,2} \xi_i v_i^\top)^\top
                + (\sum_{i}M_{i,2} \xi_i v_i^\top) M_3 (\sum_{i} M_{i,1} B_W v_i v_i^\top)^\top (M_{i,1})^\top}_\text{Noise}\\
        & \leq \frac{1.1}{0.9} \kappa_X M_1 B_W (\sum_{i} v_iv_i^\top) M_3 (\sum_{i} v_iv_i^\top) B_W^\top M_1^\top + \text{Noise}\\
        \hat{B}_W \hat{B}_W^\top
        & \geq \frac{0.9}{1.1} \frac{1}{\kappa_X} M_1 B_W (\sum_{i} v_iv_i^\top) M_3 (\sum_{i} v_iv_i^\top) B_W^\top M_1^\top + \text{Noise}
    \end{align*}
    \textcolor{red}{Noise is not right}
    where the last inequality comes from Claim \textcolor{red}{?}. By using the assumption on the estimation guarantees on $B_W (\sum_{i} v_iv_i^\top) M_3 (\sum_{i} v_iv_i^\top) B_W^\top$, we get the final bound.
\end{proof}

\begin{lemma}
    Let $\dot{B}_W = B_W \dot{V} \dot{V}^\top$. For any arbitrary $w_0$, we define
    \begin{align*}
        & \|\nu^*\|_2 = \argmin \|\nu\|_2
        \text{ s.t. }
        B_X \nu = B_W w_0 \\
        & \|\dot{\nu}\|_2 = \argmin \|\nu\|_2
        \text{ s.t. }
        \dot{B}_X \nu = B_W w_0.
    \end{align*}   
    Then, as long as $ \frac{1}{c} I_k \leq V^\top \dot{V} \leq c I_k$ for some constant $c$, we have $\|\dot{\nu}\|_2 \leq \order(\|\nu^*\|_2)$.
\end{lemma}
\begin{proof}
    By applying svd decomposition, we have $B_X = UDV^\top$ and $\dot{B}_X = UDV^\top \dot{V} \dot{V}^\top$, then by definition, we have
    \begin{align*}
        UDV^\top \dot{V} \dot{V}^\top \dot{V} \dot{\lambda}
        = UDV^\top V \lambda^*.
    \end{align*}
    where $\nu^* = V^* \lambda^*, \dot{\nu} = \dot{V} \dot{\lambda}$. Given $\lambda_{\min}(D) \geq 1$, it can be further arranged to
    \begin{align*}
        \dot{\lambda} = V^\top \dot{V} \lambda^*
    \end{align*}
    Therefore, $\|\dot{\nu}\| = \|\dot{\lambda}\| \leq \|V^\top \dot{V} \lambda^*\| \leq \order(\|\nu^*\|)$.
\end{proof}


\subsection{Main results}
e get the guarantees on $\hat{B}_W^0$ by using MLLAM proposed in \cite{thekumparampil2021sample}, as restated below, 
\begin{theorem}[Modified of Theorem 1 \cite{thekumparampil2021sample}]
For total $d_W$ linear regression tasks, each with $n_0$ samples satisfying Assumptions~\ref{ass: isotropic input},
\begin{align*}
    & n_0 \geq \widetilde{\Omega}\left(\left(1+k\left(1 / \sigma_{\min}(B_W)\right)^2\right) k \log t+k^2\right)\\
    & n_0 d_W \geq \widetilde{\Omega}\left(\left(1+\left(1 /  \sigma_{\min}(B_W)\right)^2\right)\left( \sigma_{\max}(B_W)^2 / \sigma_{\min}(B_W)^2\right) \mu d_X k^2\right)
\end{align*}
Then MLLAM, initialized at $B_{W,\mathrm{init}}$ s.t. $\left\|\left(\mathbf{I}-B_W\left(B_W\right)^{\top}\right) B_{W,\mathrm{init}}\right\|_F \leq \min \left(3 / 4, O\left(\sigma_{\max}(B_W) / \sigma_{\min}(B_W)\right)\right)$ and run for $K = \left\lceil\log _2\left(\sigma_{\max}(B_W)^2 / \sigma_{\min}(B_W) m t / \lambda_1^* \mu d_X k^2\right)\right\rceil$ iterations, outputs $B_W$ so that the following holds $\left(w . p\right.$. $\left.\geq 1-K /(d k)^{10}\right)$ :
\begin{align*}
    &\sin(\hat{B}_W, \hat{B}_W^0) \textcolor{red}{??}
    &\leq \left\|\left(\mathbf{I}-B_W\left(B_W\right)^{\top}\right)\hat{B}_W^0\right\|_F
    &\leq \widetilde{O}\left(\left(\frac{1}{\sigma_{\min}(B_W)}\right) k \sqrt{\frac{\mu d_X}{d_W n_0}}\right)
\end{align*}
\end{theorem}

Now we are ready to upper bound the estimation error $\|B_W^0 - \hat{B}_W^0\|$. From \cite{chen2022active}, we get that the explicit form of $\hat{w}(w)$, which is the estimation of actual $B_W w$ as
\begin{align*}
    \left(\hat{B}_X X_w^\top X_w \hat{B}_X^\top\right)^{-1} \hat{B}_X X_w^\top X_w B_X^\top B_W w
        + \left(\hat{B}_X X_w^\top X_w \hat{B}_X^\top\right)^{-1} \hat{B}_W X_w^\top \xi_w
\end{align*}
By abusing notation a little bit, here we use subscription $i$ to denote the items that associate the task encoded by $v_i$. Therefore, we have the upper bound for $\| B_W v_i-  \hat{B}_W v_i \|$ as
\begin{align*}
     \|\left(\hat{B}_X X_w^\top X_w \hat{B}_X^\top\right)^{-1} \hat{B}_X X_w^\top X_w B_X^\top B_W v_iv_i^\top  - B_W  v_iv_i^\top\|
        + \| \sum_t \left(\hat{B}_X X_w^\top X_w \hat{B}_X^\top\right)^{-1} \hat{B}_W X_t^\top \xi_t \nu_t^\top\|
\end{align*}
Note that the first part is only related to the source tasks while the second part is related to the target source because we also need to calculate $B_W w_0$.


{\color{red}
\textbf{To bound the first term.}
\begin{align*}     
    & \|\left(\hat{B}_X  \hat{B}_X^\top\right)^{-1} \hat{B}_X B_X^\top B_W \sum_{i=1}^{m} v_i v_i^\top - B_W \|\\
    & = \| \left(\hat{B}_X  \hat{B}_X^\top\right)^{-1} \hat{B}_X  \left(\hat{B}_X^\top \hat{B}_X + \hat{B}_{X,\perp}^\top \hat{B}_{X,\perp}\right)  B_X^\top B_W - B_W \| \\
    & \leq \|\left( \hat{B}_X B_X^\top - I_{k}\right) B_W \|
        + \|\left(\hat{B}_X  \hat{B}_X^\top\right)^{-1} \hat{B}_X \hat{B}_{X,\perp}^\top \hat{B}_{X,\perp} B_X^\top B_W \|\\
    & \leq \|B_W\| \left(\|\hat{B}_X B_X^\top - I_{k} \| +  \|\left(\hat{B}_X \hat{B}_X^\top\right)^{-1} \hat{B}_X \hat{B}_{X,\perp}^\top \hat{B}_{X,\perp} B_X^\top\|\right)\\
    & \leq  \order\left( \frac{k}{\sigma_{\min}(B_W)}\sqrt{d_X \log n }\right)\epsilon^{\frac{p}{2}} \|B_W\|
\end{align*}

where the last inequality comes from Lemma~\ref{lem: rep learning 1} and Lemma~\ref{lem: rep learning 2}.

\textbf{Secondly, we are going to  the estimation error for $B_W$ that comes from the noise $\xi$.}
Again from Lemma 18 in \cite{tripuraneni2021provable}, we have
\begin{align*}
    \| \left(\hat{B}_X X_t^\top X_t \hat{B}_X^\top\right)^{-1} \hat{B}_W X_t^\top \xi_t\|
    \leq O\left( \sqrt{\frac{k \log n}{C_{\min }}} \sqrt{k} \epsilon^{\frac{p}{2}}\right)
\end{align*}
Therefore, since all $\nu_t$ are orthonormal, as long as the target task has $n_0 \geq \frac{1}{d_W\epsilon^p}$ we still have
\begin{align*}
    \| \sum_t \left(\hat{B}_X X_t^\top X_t \hat{B}_X^\top\right)^{-1} \hat{B}_W X_t^\top \xi_t \nu_t^\top\|
    \leq O\left( \sqrt{\frac{k \log n}{C_{\min }}} \sqrt{k} \epsilon^{\frac{p}{2}}\right)
\end{align*}
}





==> Results1-CubeSpace/Analysis-general.tex <==
\subsection{Main analysis -- general}

\textcolor{red}{Wrong !!!}

Here we consider any fixed epoch $j$. For convenience, we omit the subscript $j$.

\subsubsection{Part 1}
Recall that we define $W'$ satisfying $WW' = \Tilde{W}\Tilde{W}^\top {\color{red}?}$
\begin{align*}
    & \E_{w_0 \sim \nu_0}\left[(B_W w_0)^\top \square B_W w_0\right] \\
    & = \underbrace{\E_{w_0 \sim \nu_0}(\left[(B_W w_0)^\top \square B_W w_0\right] -  \trace\left( \Tilde{\beta} \square B_W W (W')^\top B_W^\top \right)}_\text{exploration error} +  \underbrace{ \Tilde{\beta} \trace\left( \square B_W W (W')^\top B_W^\top\right)}_\text{exploitation error} 
\end{align*}
\textbf{We first deal with the exploitation error}. 
It is easy see that 
\begin{align*}
    & \Tilde{\beta} \trace\left( \square B_W \Sigma_\gamma B_W^\top\right)\\
    & =  \Tilde{\beta}\trace\left( \left(B_W \sum_{w} q_1(w)\epsilon^{-p} w w^\top (B_W)^\top 
        + B_W \sum_{w} q_2(w)\epsilon^{-q} w w^\top (B_W)^\top \right)^{-1} B_W \Sigma_\gamma B_W^\top \right)\\
    & \leq \trace\left( \left( {\color{red}?} B_W \epsilon^{-q} \tilde{W} \tilde{W}^\top (B_W)^\top \right)^{-1} B_W W (W')^\top B_W^\top \right) \\
    & = \epsilon^q \text{rank}(B_W \Tilde{W} (B_W \Tilde{W})^\top) \\
    & \leq \epsilon^q \text{rank}(\Tilde{W} \Tilde{W}^\top) \\
    & \leq \epsilon^q {\color{red} \text{rank}(\hat{B}_W \Tilde{W} \Tilde{W}^\top \hat{B}_W^\top) ??}
\end{align*}
This suggests if we corrected found the most relevant $\hat{w}_i$, then we can get $\epsilon^2$ accuracy.

% \textbf{We then deal with the exploration term.} Firstly, we have written
% \begin{align*}
%     & \E_{w_0 \sim \nu_0}\left[(B_W w_0)^\top \square B_W w_0\right] -  \Tilde{\beta}\trace\left((B_W W')^\top \square B_W W' \right) \\
%     & = \E_{w_0 \sim \nu_0}\trace\left(\square \left(B_W w_0(B_W w_0)^\top - 4\kappa_X \hat{B}_W w_0(\hat{B}_W w_0)^\top\right)\right) \\
%         & \quad + \E_{w_0 \sim \nu_0}\trace\left(\square \left(  \frac{1}{2\kappa_X}\Tilde{\beta}\hat{B}_W w'(\hat{B}_W w')^\top -  \Tilde{\beta}B_W w'(B_W w')^\top\right)\right) \\
%         & \quad + \E_{w_0 \sim \nu_0}\trace\left(\square \left( 4\kappa_X \hat{B}_W w_0(\hat{B}_W w_0)^\top -  \frac{1}{2\kappa_X}\Tilde{\beta}\hat{B}_W W'(\hat{B}_W W')^\top\right)\right)\\
%     & \leq \E_{w_0 \sim \nu_0}\trace\left(\square \left(B_W w_0(B_W w_0)^\top - 4\kappa_X \hat{B}_W w_0(\hat{B}_W w_0)^\top\right)\right) \\
%         & \quad + \Tilde{\beta}\trace\left(\square \left(  \frac{1}{2\kappa_X}\hat{B}_W W'(\hat{B}_W W')^\top -  B_W W'(B_W W')^\top\right)\right) + k \overline{\gamma} \\
%      & \leq E_{w_0 \sim \nu_0}\trace\left(\square \left(B_W w_0(B_W w_0)^\top -  M_1 B_W  w_0 w_0^\top  B_W^\top M_1^\top - \text{Noise}\right)\right) \\
%         & \quad +  \Tilde{\beta}\trace\left(\square \left(  M_1 B_W W' (W')^\top  B_W^\top M_1^\top+ \text{Noise} -  B_W W'(B_W W')^\top\right)\right) + k \overline{\gamma}\\
% \end{align*}

==> Results1-CubeSpace/Analysis-multiTarget.tex <==
\subsection{Main analysis -- multi-target}
Here we consider any fixed epoch $j$. For convenience, we omit the subscript $j$.

\subsubsection{Part 1}
\begin{align*}
    & \E_{w_0 \sim \nu_0}\left[(B_W w_0)^\top \square B_W w_0\right] \\
    & = \underbrace{\E_{w_0 \sim \nu_0}(\left[(B_W w_0)^\top \square B_W w_0\right] -  \trace\left( \Tilde{\beta}(B_W W')^\top \square B_W W' \right)}_\text{exploration error} +   \Tilde{\beta} \underbrace{\trace\left( (B_W W')^\top \square B_W W'\right)}_\text{exploitation error} 
\end{align*}
\textbf{We first deal with the exploitation error}. 
It is easy see that 
\begin{align*}
    & \Tilde{\beta}\trace\left((B_W W' )^\top \square B_W W' \right)\\
    & =  \Tilde{\beta}\trace\left( \left(B_W \sum_{w} q_1(w)\epsilon^{-p} w w^\top (B_W)^\top 
        + B_W \sum_{w} q_2(w)\epsilon^{-q} w w^\top (B_W)^\top \right)^{-1} B_W W' (B_W W')^\top \right)\\
    & \leq \trace\left( \left(  \max_i  \|\Tilde{W}(i)\|_{2(\infty)}^2 B_W \epsilon^{-q} \tilde{W} \tilde{W}^\top (B_W)^\top \right)^{-1} B_W W' (B_W W')^\top \right) \\
    & \leq \trace\left(  \left(  B_W \epsilon^{-q} W' (W')^\top (B_W)^\top \right)^{-1} B_W W' (B_W W')^\top \right) \\
    & = \epsilon^q \text{rank}(B_W W' (B_W W')^\top) \\
    & \leq \epsilon^q \text{rank}(\Tilde{W} \Tilde{W}^\top) \\
    & = \epsilon^q \text{rank}(\hat{B}_W W' (W')^\top \hat{B}_W^\top) 
\end{align*}
where the last equality comes from the definition of $W'$.

This suggests if we corrected found the most relevant $\hat{w}_i$, then we can get $\epsilon^2$ accuracy.

\textbf{We then deal with the exploration term.} Firstly, we have written
\begin{align*}
    & \E_{w_0 \sim \nu_0}\left[(B_W w_0)^\top \square B_W w_0\right] -  \Tilde{\beta}\trace\left((B_W W')^\top \square B_W W' \right) \\
    & = \E_{w_0 \sim \nu_0}\trace\left(\square \left(B_W w_0(B_W w_0)^\top - 4\kappa_X \hat{B}_W w_0(\hat{B}_W w_0)^\top\right)\right) \\
        & \quad + \E_{w_0 \sim \nu_0}\trace\left(\square \left(  \frac{1}{2\kappa_X}\Tilde{\beta}\hat{B}_W w'(\hat{B}_W w')^\top -  \Tilde{\beta}B_W w'(B_W w')^\top\right)\right) \\
        & \quad + \E_{w_0 \sim \nu_0}\trace\left(\square \left( 4\kappa_X \hat{B}_W w_0(\hat{B}_W w_0)^\top -  \frac{1}{2\kappa_X}\Tilde{\beta}\hat{B}_W W'(\hat{B}_W W')^\top\right)\right)\\
    & \leq \E_{w_0 \sim \nu_0}\trace\left(\square \left(B_W w_0(B_W w_0)^\top - 4\kappa_X \hat{B}_W w_0(\hat{B}_W w_0)^\top\right)\right) \\
        & \quad + \Tilde{\beta}\trace\left(\square \left(  \frac{1}{2\kappa_X}\hat{B}_W W'(\hat{B}_W W')^\top -  B_W W'(B_W W')^\top\right)\right) + k \overline{\gamma} \\
     & \leq E_{w_0 \sim \nu_0}\trace\left(\square \left(B_W w_0(B_W w_0)^\top -  M_1 B_W  w_0 w_0^\top  B_W^\top M_1^\top - \text{Noise}\right)\right) \\
        & \quad +  \Tilde{\beta}\trace\left(\square \left(  M_1 B_W W' (W')^\top  B_W^\top M_1^\top+ \text{Noise} -  B_W W'(B_W W')^\top\right)\right) + k \overline{\gamma}\\
\end{align*}
where the first inequality comes from the definition of $W'$ and the last inequality again comes from Lemma~\ref{lem: main base est}. 

==> Results1-CubeSpace/Analysis-singleTarget.tex <==
\subsection{Main analysis -- single target}
Here we consider any fixed epoch $j$. For convenience, we omit the subscript $j$.

\subsubsection{Part 1}
\begin{align*}
    & (B_W w_0)^\top \square B_W w_0 \\
    & = \underbrace{(B_W w_0)^\top \square B_W w_0 -  \Tilde{\beta}(B_W w')^\top \square B_W w' }_\text{exploration error} +   \Tilde{\beta} \underbrace{(B_W w')^\top \square B_W w'}_\text{exploitation error} 
\end{align*}
\textbf{We first deal with the exploitation error}. 
It is easy see that 
\begin{align*}
    & \Tilde{\beta}(B_W w' )^\top \square B_W w' \\
    & =  \Tilde{\beta}\trace\left( \left(B_W \sum_{w} q_1(w)\epsilon^{-p} w w^\top (B_W)^\top 
        + B_W \sum_{w} q_2(w)\epsilon^{-q} w w^\top (B_W)^\top \right)^{-1} B_W w' (B_W w')^\top \right)\\
    & \leq \trace\left( \left(  \|w'\|_{2 (\infty)}^2B_W \epsilon^{-q} \tilde{w} \tilde{w}^\top (B_W)^\top \right)^{-1} B_W w' (B_W w')^\top \right) \\
    & = \trace\left(  \left(  B_W \epsilon^{-q} w' (w')^\top (B_W)^\top \right)^{-1} B_W w' (B_W w')^\top \right)
    = \epsilon^q
\end{align*}
This suggests if we corrected found the most relevant $\hat{w}_i$, then we can get $\epsilon^2$ accuracy.

% \textbf{We first deal with the exploitation error}. By using the Sherman–Morrison formula, we have 
% \begin{align*}
%     \square
%     & = \left(B_W \sum_{w} q_1(w)\epsilon^{-p} w w^\top (B_W)^\top 
%         + B_W \sum_{w} q_2(w)\epsilon^{-q} w w^\top (B_W)^\top \right)^{-1}\\
%     & = \left( \frac{\epsilon^{-p}}{k_\text{explore}} \left(B_W (B_W)^\top + \Delta_W \right)+ \epsilon^{-q}B_W \hat{w}_i (B_W \hat{w}_i)^\top \right)^{-1}\\
%     & = \epsilon^p k_\text{explore} \left( B_W (B_W)^\top + \Delta_W \right)^{-1}
%         - \frac{\epsilon^{2p-q} k_\text{explore}^2  \left( B_W (B_W)^\top + \Delta_W \right)^{-1} B_W \hat{w}_i (B_w \hat{w}_i)^\top  \left( B_W (B_W)^\top + \Delta_W \right)^{-1}}{1 + k_\text{explore} \epsilon^{p-q}  (B_w \hat{w}_i)^\top  \left( B_W (B_W)^\top + \Delta_W \right)^{-1} B_W \hat{w}_i}
% \end{align*}
% Therefore, let $(B_W \hat{w}_i)^\top  \left( B_W (B_W)^\top + \Delta_W \right)^{-1} B_W \hat{w}_i = \square_2$, which is a scalar there, then we have
% \begin{align*}
%     (B_W \hat{w}_i)^\top \square B_W \hat{w}_i 
%     & = \epsilon^p d_W \square_2 - \frac{\epsilon^{2p-q} d_W^2 \square_2 \square_2}{1 + d_W \epsilon^{p-q} \square_2} \\
%     & = \frac{\epsilon^p k_\text{explore} \square_2 + \epsilon^{2p-q} k_\text{explore}^2 \square_2 \square_2 - \epsilon^{2p-q} k_\text{explore}^2 \square_2 \square_2}{1 + k_\text{explore} \epsilon^{p-q} \square_2}\\
%     & \leq \epsilon^{q}
% \end{align*}

\textbf{We then deal with the exploration term.} Firstly, we have written
\begin{align*}
    & (B_W w_0)^\top \square B_W w_0 -  \Tilde{\beta}(B_W w')^\top \square B_W w' \\
    & = \trace\left(\square \left(B_W w_0(B_W w_0)^\top - 4\kappa_X \hat{B}_W w_0(\hat{B}_W w_0)^\top\right)\right) 
        + \trace\left(\square \left(  \frac{1}{2\kappa_X}\Tilde{\beta}\hat{B}_W w'(\hat{B}_W w')^\top -  \Tilde{\beta}B_W w'(B_W w')^\top\right)\right) \\
        & \quad + \trace\left(\square \left( 4\kappa_X \hat{B}_W w_0(\hat{B}_W w_0)^\top -  \frac{1}{2\kappa_X}\Tilde{\beta}\hat{B}_W w'(\hat{B}_W w')^\top\right)\right)\\
    & \leq \trace\left(\square \left(B_W w_0(B_W w_0)^\top - 4\kappa_X \hat{B}_W w_0(\hat{B}_W w_0)^\top\right)\right) 
        + \Tilde{\beta} \trace\left(\square \left(  \frac{1}{2\kappa_X}\hat{B}_W w'(\hat{B}_W w')^\top -  B_W w'(B_W w')^\top\right)\right) \\
     & \leq \trace\left(\square \left(B_W w_0(B_W w_0)^\top -  M_1 B_W  w_0 w_0^\top  B_W^\top M_1^\top - \text{Noise}\right)\right) \\
        &  \quad + \Tilde{\beta} \trace\left(\square \left(  M_1 B_W w' w'^\top  B_W^\top M_1^\top+ \text{Noise} -  B_W w'(B_W w')^\top\right)\right) \\
\end{align*}
where the first inequality comes from the definition of $w', \tilde{\beta}$ and the last inequality comes from Lemma~\ref{lem: main base est}. We can further upper bound the above by
\begin{align*}
    & 2\|\square\|_2\|\text{Noise}\| 
        + \|\square\|_2 \left(\|w_0\| + \|w'\|\right)\|B_W B_W^\top - M_1 B_W  B_W^\top M_1^\top\| \\
    & \leq 2\frac{\epsilon^p k_\text{explore}}{\sigma_{\min}^2(B_W)}\|\text{Noise}\| 
        + \frac{\epsilon^p k_\text{explore}}{\sigma_{\min}^2(B_W)} \left(\|w_0\| + \|w'\|\right)\|B_W B_W^\top - M_1 B_W  B_W^\top M_1^\top\|
\end{align*}

\paragraph{Combine exploration and exploitation} Now we have
\begin{align*}
    (B_W w_0)^\top \square B_W w_0
    & \leq \epsilon^{q} 
    + 2\epsilon^p k_\text{explore}\|\text{Noise}\| 
        + \epsilon^p k_\text{explore} \left(\|w_0\| + \|\hat{w}_i\|\right)\|B_W B_W^\top - M_1 B_W  B_W^\top M_1^\top\|
\end{align*}

Now we want to further upper bound the second term to ensure that, our overall estimation to $B_W$ has error $\otil(\epsilon^{q-p})$ so that the second term can again be upper bound by $\otil(\epsilon^q)$.

\iffalse
\subsubsection{Part 2}

Now we are ready to bound $\|B_W B_W^\top - M_1 B_W  B_W^\top M_1^\top\|$, it can be further decomposed as
\begin{align*}
    & \| \left( M_1 B_W  B_W^\top M_1^\top - B_WB_W^\top + \text{Noise} \right) \| \\
    & = \| \left( \left(M_1 B_W + \sum_{i} M_{i,2} \xi_i v_i^\top \right) \left(M_1 B_W + \sum_{i} M_{i,2} \xi_i v_i^\top \right)^\top - B_WB_W^\top \right) \| \\
    & \leq \left\|\left(M_1 B_W + \sum_{i} M_{i,2} \xi_i v_i^\top \right) - B_W \right\|
    \left( \|(M_1 B_W + \sum_{i} M_{i,2} \xi_i v_i^\top\| + \|B_W\| \right) \\
    & \leq \left\|\left(M_1 B_W + \sum_{i} M_{i,2} \xi_i v_i^\top \right) - B_W \right\| \left(2\|B_W\| + \left\|\left(M_1 B_W + \sum_{i} M_{i,2} \xi_i v_i^\top \right) - B_W \right\|\right)
\end{align*}
Replace the definition of $M_1, M_{i,2}$, we can further bound $\left\|\left(M_1 B_W + \sum_{i} M_{i,2} \xi_i v_i^\top \right) - B_W \right\|$ as
\begin{align*}
     \left( \left\|\left(\hat{B}_X \hat{B}_X^\top\right)^{-1} \hat{B}_X  B_X^\top B_W w \right\|
        + \left\| \sum_{i=0}^k \left(\hat{B}_X X_i^\top X_i \hat{B}_X^\top\right)^{-1} \hat{B}_W X_i^\top \xi_i \nu_i^\top \right\|\right)  \max_{B_W \in \calB_W}\sigma_{max}(B_W) 
\end{align*}
Note that the first part is only related to the source tasks while the second part is related to the target source because we also need to calculate $B_W w_0$

\textbf{To bound the first term.}
By using the regularized ERM algorithm propose in \cite{tripuraneni2020theory}, we get 
\begin{align*}
    \sin(\hat{B}_X, \hat{B}_X)
    & \leq \order\left( \sqrt{\frac{k}{\sigma_{\min}(B_W \sum_{i=0}^{k} \nu_i \nu_i^\top B_W^\top)} }\sqrt{\max\{d_X,T\}k (\log n) \epsilon^{p}}\right) \\
    &\leq \order\left( \frac{k}{\sigma_{\min}(B_W)}\sqrt{d_X (\log n) \epsilon^{p}}\right)
\end{align*}
We refer the details into \textcolor{red}{?}. Combining these two results, we are ready to show the estimation error for $B_W$ that comes from the $B_X$ estimation.

\begin{align*}     
    & \|\left(\hat{B}_X  \hat{B}_X^\top\right)^{-1} \hat{B}_X B_X^\top B_W \sum_{i=1}^{m} v_i v_i^\top - B_W \|\\
    & = \| \left(\hat{B}_X  \hat{B}_X^\top\right)^{-1} \hat{B}_X  \left(\hat{B}_X^\top \hat{B}_X + \hat{B}_{X,\perp}^\top \hat{B}_{X,\perp}\right)  B_X^\top B_W - B_W \| \\
    & \leq \|\left( \hat{B}_X B_X^\top - I_{k}\right) B_W \|
        + \|\left(\hat{B}_X  \hat{B}_X^\top\right)^{-1} \hat{B}_X \hat{B}_{X,\perp}^\top \hat{B}_{X,\perp} B_X^\top B_W \|\\
    & \leq \|B_W\| \left(\|\hat{B}_X B_X^\top - I_{k} \| +  \|\left(\hat{B}_X \hat{B}_X^\top\right)^{-1} \hat{B}_X \hat{B}_{X,\perp}^\top \hat{B}_{X,\perp} B_X^\top\|\right)\\
    & \leq  \order\left( \frac{k}{\sigma_{\min}(B_W)}\sqrt{d_X \log n }\right)\epsilon^{\frac{p}{2}} \|B_W\|
\end{align*}

where the last inequality comes from Lemma~\ref{lem: rep learning 1} and Lemma~\ref{lem: rep learning 2}.

\textbf{Secondly, we are going to  the estimation error for $B_W$ that comes from the noise $\xi$.}
Again from Lemma 18 in \cite{tripuraneni2021provable}, we have
\begin{align*}
    \| \left(\hat{B}_X X_t^\top X_t \hat{B}_X^\top\right)^{-1} \hat{B}_W X_t^\top \xi_t\|
    \leq O\left( \sqrt{\frac{k \log n}{C_{\min }}} \sqrt{k} \epsilon^{\frac{p}{2}}\right)
\end{align*}
Therefore, since all $\nu_t$ are orthonormal, as long as the target task has $n_0 \geq \frac{1}{d_W\epsilon^p}$ we still have
\begin{align*}
    \| \sum_t \left(\hat{B}_X X_t^\top X_t \hat{B}_X^\top\right)^{-1} \hat{B}_W X_t^\top \xi_t \nu_t^\top\|
    \leq O\left( \sqrt{\frac{k \log n}{C_{\min }}} \sqrt{k} \epsilon^{\frac{p}{2}}\right)
\end{align*}
\fi 
\subsubsection{Part 3}
Combine the results from part 1 and part 2, we have
\begin{align*}
    & (B_W w_0)^\top \square B_W w_0 \\
    & \leq \epsilon^{q} 
    + \epsilon^p k \frac{1}{\sigma_{\min}^2(B_W)} \left( \|w_0\| + \|\hat{w}_i\|\right)
    \order\left( \frac{k}{\sigma_{\min}(B_W)}\sqrt{d_X\log n }\right)\epsilon^{\frac{p}{2}} \|B_W\| \\
    & \leq \epsilon^{q} 
    + \epsilon^{\frac{3p}{2}} \underbrace{k^{\frac{3}{2}} \frac{\sigma_{max}(B_W)}{\sigma_{\min}^3(B_W)} \left( \|w_0\| + \|\hat{w}_i\|\right) \sqrt{\max\{d_X,T\}\log n }}_{C^*}
\end{align*}

Now we have sampled $k + 1$ number of tasks, where $k$ tasks come from the exploration part and one comes from the exploration. Denote $\Tilde{W}_\calS = \{\sqrt{n_t} w_t \}_{t=0}^{k}$, by using the result in \cite{chen2022active}, we have 
\begin{align*}
    \textsc{ER}(\hat{B},\hat{w}_{M+1})
    &\leq \frac{\|P_{X_0\hat{B}}^{\bot}X_{M+1}B_X B_W w_0\|^2}{n_{M+1}} +\sigma^2\frac{k + \log(1/\delta)}{n_0}
\end{align*}
Decompose $B_W \Tilde{W}_\calS (B_W \Tilde{W}_\calS)^\top$ as $UDU^\top$ and let $\Sigma_W = U\sqrt{D}U^\top$. So we can upper-bound key terms as
\begin{align*}
    &\|P_{X_0\hat{B}}^{\bot}X_{M+1}B_X B_W w_0\|^2 \\
    & = \|P_{X_0\hat{B}}^{\bot}X_{M+1}B_X \Sigma_W^{\frac{1}{2}} \Sigma_W^{- \frac{1}{2}} B_W w_0\|^2 \\
    & \leq \|P_{X_0\hat{B}}^{\bot}X_{M+1}B_X \Sigma_W^{\frac{1}{2}}\|_F^2 \|\Sigma_W^{- \frac{1}{2}} B_W w_0\|^2 \\
    & = \|P_{X_0\hat{B}}^{\bot}X_{M+1}B_X B_W \tilde{W}_\calS\|_F^2 (B_W w_0)^\top \left( B_W \tilde{W}_\calS \tilde{W}_\calS^\top B_W ^\top \right)^{-1} B_W w_0 \\
    & =  \|P_{X_0\hat{B}}^{\bot}X_{M+1}B_X B_W \tilde{W}_\calS\|_F^2 (B_W w_0)^\top
        (B_W w_0)^\top \square B_W w_0 \\
    & \lessapprox \sigma^2 \left(kd_X\log( (\kappa N_i )/d_W) + \log\frac{1}{\delta} \right)
        \left(\epsilon^q + \epsilon^{\frac{3p}{2}}C^*\right)
\end{align*}
The first comes from standard passive learning results and the second one has been bounded above.

\textcolor{red}{Find the optimal $p$ given $q$}

\subsection{Upper bound for $\|w'\|$}

From Line 12, we know the sample complexity scales with $\|w'\|_{2(\infty)}$, which is the projection penalty. Now we have for any norm, 
\begin{align*}
    \|\hat{B}_W^j w'\|
    = \|\hat{B}_W^j w_0\|
    \leq \| (\hat{B}_W^j - B_W) w_0 \| + \|B_W w_0\| 
    \leq 2 \|B_W w_0\| 
\end{align*}
and 
\begin{align*}
    \|\hat{B}_W^j w'\| \geq \frac{1}{2}\|B_W w'\| 
\end{align*}
\textcolor{red}{Because $w' \perp w_0$, so that $B_W$ is not important.}
Based on the assumption that $\|B_W(j)\| = \Theta(1)$ for any $j$-th column and the closeness of between $B_W, \hat{B}_W^j$ \text{color}{TODO}, we have
\begin{align*}
    \|w'\|_2 \leq \frac{1}{\sigma_{\min}^2(B_W)}\|B_W w'\|_2
    & \leq \frac{1}{\sigma_{\min}^2(B_W)}\|B_W w'\|_2 \\
    & \leq \frac{4}{\sigma_{\min}^2(B_W)} \|B_W w_0\|_2 
\end{align*}
and
\begin{align*}
    \|w'\|_\infty \leq \|w'\|_2 \leq \frac{4}{\sigma_{\min}^2(B_W)} \|B_W w_0\|_2
\end{align*}
% \begin{align*}
%    \|w'\|_\infty 
%     & \leq \min\left\{ \frac{\sqrt{d_W}}{\sigma_{\min}^2(B_W)} \|B_W w'\|_0, \|w'\|_2 \right\} \\
%     & \leq \min\left\{ \frac{4\sqrt{d_W}}{\sigma_{\min}^2(B_W)} \|B_W w_0\|_0,  \quad \frac{4}{\sigma_{\min}^2(B_W)} \|B_W w_0\|_2 \right\}
% \end{align*}

\subsubsection{Auxiliary Lemmas}

\begin{lemma}
\label{lem: rep learning 1}
\begin{align*}
     \|I_{k}  - \hat{B}_X B_X^\top\|
     \leq \order\left( \sqrt{k} \sin(\hat{B}_X, \hat{B}_X)\right)
\end{align*}
\end{lemma}
\begin{proof}
    Denote $B_X \hat{B}_X^\top  = UDV^\top$, by definition, we have
    $D = \text{diag}(\cos{\theta_1}, \cos{\theta_2}, \ldots, \cos{\theta_k})$ from the largest singular value to minimum singular value and
    $\sin{\theta_k} \leq \sin(\hat{B}_X, \hat{B}_X)$. Therefore we have,
    \begin{align*}
       \text{Tr}(\hat{B}_X B_X^\top) 
       \geq k \sqrt{1- \sin^2(\hat{B}_X, \hat{B}_X)}
       \geq k - k \sin^2(\hat{B}_X, \hat{B}_X)
    \end{align*}
    And 
    \begin{align*}
        \|I_{k}  - \hat{B}_X B_X^\top\|^2
        & =  \lambda_{\max} \left(\left(I_{k}  - \hat{B}_X B_X^\top\right)^\top \left(I_{k}  - \hat{B}_X B_X^\top\right)\right)\\
        % & \leq \trace \left(I_{k}  - \hat{B}_X B_X^\top\right)^\top \left(I_{k}  - \hat{B}_X B_X^\top\right)\\
        & \leq \lambda_{\max} \left( I_k + \left(\hat{B}_X B_X^\top\right)^\top \hat{B}_X B_X^\top
        - \left(\hat{B}_X B_X^\top\right)^\top -  \hat{B}_X B_X^\top\right) \\
        & \leq 2\sin^2(\hat{B}_X, B_X)
    \end{align*}
\end{proof}

\begin{lemma}[Restate from \cite{tripuraneni2021provable}]
\label{lem: rep learning 2}
    Given $\sin(\hat{B}_X, \hat{B}_X) \leq \order\left( \frac{1}{\sqrt{\nu}} \sqrt{\max\{d_X,T\}k\log n }\epsilon^{\frac{p}{2}}\right)$, and $\hat{B}_X, B_X$ are orthonormal matrices, as well as $\E[x x^T] = I_{d_X}$ for all tasks $w$, we have
    \begin{align*}
        \|\left(\hat{B}_X X_w^\top X_w \hat{B}_X^\top\right)^{-1} \hat{B}_X X_w^\top X_w \hat{B}_{X,\perp}^\top \hat{B}_{X,\perp} B_X^\top\|
        \leq \order\left( \frac{1}{\sqrt{\nu}} \sqrt{\max\{d_X,T\}k\log n }\epsilon^{-\frac{p}{2}}\right)
    \end{align*}
\end{lemma}
\begin{proof}
    Here we follow the same proof step as in \cite{tripuraneni2021provable}.
    \begin{align*}
        &\|\left(\hat{B}_X X_w^\top X_w \hat{B}_X^\top\right)^{-1} \hat{B}_X X_w^\top X_w \hat{B}_{X,\perp}^\top \hat{B}_{X,\perp} B_X^\top\| \\
        & \leq \|\left(\hat{B}_X X_w^\top X_w \hat{B}_X^\top\right)^{-1} \hat{B}_X X_w^\top X_w \hat{B}_{X,\perp}^\top \| \sin(\hat{B}_X, \hat{B}_X) \\
        & \leq C_\text{condi} \sin(\hat{B}_X, \hat{B}_X)
    \end{align*}
    where $C_\text{condi} = C_\text{max}/C_\text{min}$ = 1 in this case.
\end{proof}


\begin{lemma}
\label{lem: explore model est}
    As long as $\Delta \geq -\frac{1}{\sigma_{\min}^2}I_k$, we have
    \begin{align*}
        \left( BB^\top + \Delta \right)^{-1} \leq 2(BB^\top)^{-1}
    \end{align*}
\end{lemma}
\begin{proof}
    Let $\Delta_W = UDV^\top$ and $D_+  = |D|$,  using woodbury inequality, we have
    \begin{align*}
        \left( BB^\top + \Delta \right)^{-1}
        & = (BB^\top)^{-1} - (BB^\top)^{-1}U(D^{-1}+ V^\top(BB^\top)^{-1}U)^{-1}V^\top (BB^\top)^{-1}\\
        & \leq (BB^\top)^{-1} + (BB^\top)^{-1}U D_+ V^\top (BB^\top)^{-1}\\
        & \leq (BB^\top)^{-1}  \left( I_k + \frac{1}{\sigma_{\min}^2(B_W)}U D_+ V^\top \right)\\
        & \leq 2(BB^\top)^{-1}
    \end{align*}
\end{proof}

==> Results1-CubeSpace/Results1-CubeSpace.tex <==
\section{A theoretical analysis under benign $\calW_\text{source}$ setting}

\subsection{Assumption}

In this section, we mainly consider the $\calW_\text{source}$ and $\calW_\text{target}$ satisfies one of the following assumptions.

\begin{assumption}[Cubic assumption]
    We assume both the source task space and the target task space are cubic. 
    \begin{align*}
        \calW_\text{source} = [-1,1]^{d_W},
        \quad\text{and} \quad
        \calW_\text{target} = [-1,1]^{d_W+1}
    \end{align*}
    Note that the target task space is larger than the source task space so in some special cases, we have $w_0 \perp \calW_\text{source}$
\end{assumption}

\begin{assumption}[Ball assumption]
    We assume both the source task space and the target task space are ball 
    \begin{align*}
        \calW_\text{source} = \fB^{d_W}(1)
        \quad\text{and} \quad
        \calW_\text{target} = \fB^{d_W+1}(1)
    \end{align*}
    Again the target task space is larger than the source task space so in some special cases, we have $w_0 \perp \calW_\text{source}$
\end{assumption}

In addition, we also require some other assumptions

\begin{assumption}[Isotropic Gaussian Input]
\label{ass: isotropic input}
    Here we add an extra assumption on the input $x_{i,w} \sim \calN(0,I_d)$ for all $w$.
\end{assumption}

\begin{assumption}
    Each column of $B_W$ has magnitude $\Theta(1)$
\end{assumption}


\input{Results1-CubeSpace/Algorithm}
\input{Results1-CubeSpace/Analysis-Stage0}
\input{Results1-CubeSpace/Analysis-singleTarget}
\input{Results1-CubeSpace/Analysis-multiTarget}
\input{Results1-CubeSpace/Analysis-general}

==> other_theory.tex <==
\section{Other results}
\begin{lemma}
\label{lem: uniform case}
    When = the target task is uniformly spread $\|\E_{w_0 \sim \nu_\text{target}}B_W w_0 w_0^\top B_W^\top \| = \frac{1}{k}$ and the task representation is well-conditioned $\sigma_{\min}^2(B_W^\text{source}) = \frac{d_W}{k}$, we have
    \begin{align*}
        \|W_i^*\|_2^2 = \frac{1}{d_W}
    \end{align*}
\end{lemma}
\begin{proof}
Do a svd decomposition on the $B_W^\text{source}$ gives $\frac{T}{k} U_1 V_1^\top $. For any $i$, let $w$ satisfies
\begin{align*}
    \sqrt{\frac{d_W}{k}} U_1 V_1^\top w = \sqrt{\frac{1}{k}} u_i  
\end{align*}
Rearrange the above equality, we have
\begin{align*}
    V_1^\top w = \sqrt{\frac{1}{d_W}} U_1^\top u_i
\end{align*}
Because $W_i = \argmin \|w\|_2$ satisfy the above constraints, we have
\begin{align*}
    \|W_i^*\|_2^2 = \| V_1^\top w \|_2^2 = \left\|\sqrt{\frac{1}{d_W}} U_1^\top u_i \right\|_2^2 = \frac{1}{d_W}
\end{align*}
\end{proof}

\begin{lemma}
\label{lem: compare L_1 with L_2}
Let 
\begin{align*}
    & \nu_1 = \argmin_{\nu} \|\nu\|_1 \text{ s.t } B_W \nu = B_W w_0 \\
    & \nu_2 = \argmin_{\nu} \|\nu\|_2 \text{ s.t } B_W \nu = B_W w_0
\end{align*}
Then $\|\nu_1\|_1^2 \geq \| \nu_2\|_2^2$.
\end{lemma}
\begin{proof}
    \begin{align*}
        \|\nu_1\|_1^2 \geq \|\nu_1\|_2^2 \geq \|\nu_2\|^2
    \end{align*}
\end{proof}

==> theory-algo-archive.tex <==
\subsection{Algorithm}
\yifang{Currently I plan to only offer the target-aware theory in the main paper and postpone the target-agnostic in the appendix.}
\begin{algorithm}[H]
\caption{Target-aware algorithm for benign source space}
\label{algo: main}
\begin{algorithmic}[1]
\STATE \textbf{Inputs.} (Skip here)
\STATE Set $q_0$ as
$
    q_0(e_t) = \frac{1}{d_W}, \forall t \in d_W, \text{and} \quad q_0(w) = 0 \text{ otherwise}
$
\STATE Set $n_0 = \textcolor{red}{pending}$. Collect $n_0(w) = n_0 q_0(w)$ data for each task denoted as $\{X_w\}_{w | q(w) \neq 0}$
\STATE Update $\hat{B}_X \leftarrow \calO_\text{offline 1}^X(\{X_w\}_{w | q_0(w) \neq 0 })$ and $\hat{B}_W^\text{source} \leftarrow \calO_\text{offline 1}^W(\{X_w\}_{w | q_0(w) \neq 0 }, \hat{B}_X)$ 
\STATE Compute $q_1$ as 
$q_1(v_i) = \frac{1}{k}, \forall i \in k$, and $q_0(w) = 0$ otherwise.
\text{Here} $v_i$ is the $i$-th vector of $V$,  where $U,D,V \leftarrow \text{SVD}(\hat{B}_W^\text{source})$ 
\FOR{$j = 1,2,3, \ldots$}
    \STATE Set {\color{red}$n_1^j \approx k d_X \epsilon^{-\frac{3}{2}}$}. Collect $n_1^j(w) = n_1^j q_1(w)$ data for each task denoted as $\{X_w\}_{w | q_1(w) \neq 0}$.
    \STATE $\hat{\phi}_X \leftarrow \calO_\text{offline 2}^X(\{X_w\}_{w | q_1(w) \neq 0})$,  $\hat{B}_W^\text{source} \leftarrow \calO_\text{offline 2}^W(\{X_w\}_{w | q_1(w) \neq 0}, \hat{B}_X)$ \\
    and  $\hat{B}_W^\text{target} \leftarrow \calO_\text{offline 2}^W(\dot{X}_\text{target}, \hat{B}_X)$
    \STATE Find a set of target-aware tasks parameterized by $\Tilde{W}_j$ with each column $i$ as
    \begin{align*}
        \Tilde{W}_j(i) = \text{Proj}_{\calW_\text{source}} w_i^\prime =
        \begin{cases}
            &  \frac{w_i^\prime}{\|w_i^\prime\|_2} \quad \text{when } \calW_\text{source} = [-1,1]^{d_W} \\
            &  \frac{w_i^\prime}{\|w_i^\prime\|_\infty} \quad \text{when } \calW_\text{source} = \fB^{d_W}(1)
        \end{cases}
    \end{align*}
    where
    \begin{align*}
        \text{i-th column of } W' = 
        &w_i^\prime = 
        \begin{cases}
            & \argmin_{w} \|w\|_2 \quad \text{when } \calW_\text{source} = [-1,1]^{d_W} \\
            & \argmin_{w} \|w\|_\infty \quad \text{when } \calW_\text{source} = \fB^{d_W}(1) 
        \end{cases} \\
        \text{s.t.} \quad & \hat{B}_{W,j}^\text{source} w =  u_i\sqrt{\lambda_i} \quad {\color{red} \forall \Lambda_i \geq ?}\\
        & \text{where } U, \Lambda \leftarrow  \text{Eig}\left(\E_{w_0 \sim \nu_\text{target}}\left[\hat{B}_{W,j}^\text{target}  w_0 (\hat{B}_{W,j}^\text{target} w_0)^\top \right] \right)
    \end{align*}
    \STATE Compute $q_2^j$ as 
    $ q_2^j(w) = \frac{1}{\text{\# col}(\tilde{W}_j)}, \forall w \in \text{col}(\Tilde{W}_j)$ and $ q_2^j(w) = 0$ otherwise
    
    % \STATE Assign $n_2^j(w) \approx \frac{q_2^j(w)}{\text{\# col}(\tilde{W}_j)\epsilon^2}* {\color{red}\tilde{\beta}} \frac{\trace\left( \hat{B}_{W,j} W' \right)}{\trace\left( \hat{B}_{W,j} \text{Proj}_{\calW_\text{source}} W' \right)} $ sampling budget to each task parameterized by each column of $\Tilde{W}_j$ 
    \STATE Assign $n_2^j$ total sampling budget as
    \begin{align*} 
        \text{\# col}(\tilde{W}_j) \max_i \frac{\tilde{\beta}\Lambda_i}{\|\hat{B}_{W,j} \tilde{W}_j(i)\|_2^2} \epsilon_j^{-2} 
        = 
        \begin{cases}
            & \text{\# col}(\tilde{W}_j)\tilde{\beta} \max_i \|W_j^\prime(i)\|_2^2 \epsilon_j^{-2} \quad \text{when } \calW_\text{source} = [-1,1]^{d_W} \\
            &\text{\# col}(\tilde{W}_j)\tilde{\beta} \max_i \|W_j^\prime(i)\|_\infty^2 \epsilon_j^{-2}  \quad \text{when } \calW_\text{source} = \fB^{d_W}(1)
        \end{cases}
    \end{align*}
    \STATE Collect $n_2^j(w) = n_2^j q_2^j(w)$ data for each task denoted as $\{X_w\}_{w | \tilde{q}(w) \neq 0}$. 
    \STATE Update the model, note that both data collected from stage 2 and stage 3 are used to compute $\Tilde{B}_X$ but only the target-related subspace is used to compute $\Tilde{B}_W$, .
    \begin{align*}
        &\tilde{B}_X \leftarrow \calO_\text{offline 3}^X(\{X_w\}_{w | q_1(w) \neq 0 \text{ and } \tilde{q}(w) \neq 0}) \\
        & \tilde{B}_W^\text{target} \leftarrow \calO_\text{offline 3}^W(X_\text{target})
    \end{align*}
\ENDFOR
\STATE \textbf{Return }  $\tilde{B}_X, \tilde{B}_w^\text{source}$
\end{algorithmic}
\end{algorithm}

\yifang{Add a brief explain}

\yifang{Add choice of $\calO_\text{offline}$}

\subsection{Results}
\begin{theorem}[Source space as a ball]
    in order to let $ER \leq \varepsilon^2$ with probability $1-\delta$, the number of source samples $N_{tot}$ is at most
    \begin{align*}
        kd_X (k^*)^2 \max_i \|W'_i\|_2^2 \epsilon^{-2}
        + \text{\color{red} Low order term}
    \end{align*}
    Here $k^* = \text{rank}(\E_{w_0 \sim \nu_\text{target}}B_W w_0 w_0^\top B_W^\top)$ represents the effective dimension of target and $W_i^*$ is the solution of 
    \begin{align*}
        W^*_i = \argmin_{w \in \calW_\text{source}} \|w\|_2 
        \quad \text{s.t} \quad B_W^\text{source} w = u_i \sqrt{\lambda_i} 
        \text{ where } U, \Lambda \leftarrow \text{Eig}(\E_{w_0 \sim \nu_\text{target}}B_W w_0 w_0^\top B_W^\top).
    \end{align*}
    And the number of target samples $N_\text{target}, \dot{N}_\text{target}$ is at least
    \begin{align*}
        \yf{TODO}
    \end{align*}
\end{theorem}

\yifang{Add proof sketch if with enough space}

\paragraph{Compare with passive learning} By choosing $\{e_i\}_{i \in [d_W]}$ as a fixed source set, we reduce the problem to a discrete setting and compare it with the passive learning. In \cite{du2021fewshot}, the authors get $N_\text{total}$ as most 
\begin{align*}
    \frac{k d_X d_W \|\E_{w_0 \sim \nu_\text{target}}B_W w_0 w_0^\top B_W^\top \|}{\sigma_{\min}^2(B_W) } \epsilon^{-2}.
\end{align*}
We first consider the cases in their paper that the target task is uniformly spread $\|\E_{w_0 \sim \nu_\text{target}}B_W w_0 w_0^\top B_W^\top \| = \frac{1}{k}$.
\begin{itemize}
    \item When the task representation is well-conditioned $\sigma_{\min}^2(B_W^\text{source}) = \frac{d_W}{k}$. We have a passive one as $ \otil(k d_X \epsilon^{-2})$ while the active one $\otil(kd_X \frac{k^2}{d_W} \epsilon^{-2})$ (See Lemma~\ref{lem: uniform case} for details), which suggests as long as $d_W \gg k^2$, our active learning algorithm gain advantage even in a relatively uniform spread data and representation conditions. 
    \item Otherwise, we consider the extreme case that  $\sigma_{\min}^2(B_W^\text{source}) = 1$. We have passive one  $\otil(d_X d_W\epsilon^{-2})$ while the active one $\otil(k^2 d_X \epsilon^{-2})$.
\end{itemize}
Both of them indicate the necessity of considering the continuous case with large $d_W$ even if everything is uniformly spread. On the other hand, whether we can achieve the same result as the passive one when $d_W \leq k^2$ remains to be explored in the future.  We then consider the single target $w_0$ case.
\begin{itemize}
    \item With well-conditioned $B_W$, the passive one now has sample complexity $\order(k^2 d_X \epsilon^{-2})$ while the active gives a strictly improvement $\order(\frac{k^2 d_X}{d_W}  \epsilon^{-2})$.
    \item With ill-conditioned $B_W$ where $\sigma_{\min}(B_W) = 1$ and $\max_i \|W_i^*\| = 1$, that is, only a particular direction in source space contributes to the target. The Passive one now has sample complexity $\order(k d_X d_W \epsilon^{-2})$ while our active one only has $kd_X \epsilon^{-2}$, which demonstrates the benefits of our algorithm in unevenly distributed source space.
\end{itemize}


\paragraph{Compare with previous active learning} By using the same discrete reduction and set single target $w_0$, we compare our result with the current state-of-art active representation algorithm in \yf{ref}. They achieves $\otil(kd_X\|\nu\|_1^2 \epsilon^{-2})$, where
$\nu = \argmin_{\nu} \|\nu\|_1 \text{ s.t } B_W \nu = B_W w_0$. 
On the other hand, our active one gives $\otil(kd_X\|w^*\|_2^2 \epsilon^{-2})$, where
$w^* = \argmin_{\nu} \|nu\|_2 \text{ s.t } B_W \nu = B_W w_0$, which is strictly better than the discrete one. This again indicates the separation between continuous and discrete cases, because as discussed in \yf{ref}, for fixed discrete sets, the $L_1$ norm regularization is strictly better than $L_2$.

\paragraph{Save task number.} As we motivated in the introduction, even under the same source sample complexity, few source tasks can save the environment maintain costs and facilitate the joint training process. In our active learning algorithm, regardless of the initial warm-up stage, we only require maintaining $\otil(k + \log(N_\text{total}k^*))$ number of source tasks, where the first term comes from $q_1$ in the target-agnostic stage and the second term comes from $q_2$ in the target-aware stage. In practice, $q_1$ from the target-agnostic stage can be updated. But by setting a changing threshold, we can still keep a low task number.




% \subsubsection{Overview}
%  We first show that the excess risk highly depends on 
%  \begin{align*}
%       \trace\left(\left( B_W \tilde{W}_\calS \tilde{W}_\calS^\top B_W ^\top \right)^{-1} B_W \tilde{W}_\text{target} \tilde{W}_\text{target}^\top B_W^\top \right)
%  \end{align*}
%  where $\tilde{W}_\calS$ and $\calW_\text{target}$ are training source and target-related parameters which we will specify later.

% Denoting $\left( B_W \tilde{W}_\calS \tilde{W}_\calS^\top B_W ^\top \right)^{-1}$ as $\square$, we can further decompose it into
%  \begin{align*}
%      \underbrace{\E_{w_0 \sim \nu_0}(\left[(B_W w_0)^\top \square B_W w_0\right] -  \trace\left( \Tilde{\beta}(B_W W')^\top \square B_W W' \right)}_\text{target-agnostic exploration error} +   \Tilde{\beta} \underbrace{\trace\left( (B_W W')^\top \square B_W W'\right)}_\text{taregt-aware exploration error} 
%  \end{align*}

%  To the upper bound the target-agnostic exploration error, the key is to show the $q_1$ distribution well approximate the $k$-dim embed space. \yifang{Add more?}
 
%  Then, to upper bound the target-aware exploration error, we will firstly prove the increasingly accurate estimation on $B_X,B_W$ and then show a proper regularization that avoids over-exploration. \yifang{TODO}



